Automatically Labeling Clinical Trial Outcomes: A Large-Scale Benchmark for Drug Development

Background The cost of drug discovery and development is substantial, with clinical trial outcomes playing a critical role in regulatory approval and patient care. However, access to large-scale, high-quality clinical trial outcome data remains limited, hindering advancements in predictive modeling and evidence-based decision-making. Methods We present the Clinical Trial Outcome (CTO) benchmark, a fully reproducible, large-scale repository encompassing approximately 125,000 drug and biologics trials. CTO integrates large language model (LLM) interpretations of publications, trial phase progression tracking, sentiment analysis from news sources, stock price movements of trial sponsors, and additional trial-related metrics. Furthermore, we manually annotated a dataset of clinical trials conducted between 2020 and 2024 to enhance the quality and reliability of outcome labels. Results The trial outcome labels in the CTO benchmark agree strongly with expert annotations, achieving an F1 score of 94 for Phase 3 trials and 91 across all phases. Additionally, benchmarking standard machine learning models on our manually annotated dataset revealed distribution shifts in recent trials, underscoring the necessity of continuously updated labeling approaches. Conclusions By analyzing CTO's performance on recent clinical trials, we demonstrate the ongoing need for high-quality, up-to-date trial outcome labels. We publicly release the CTO knowledge base and annotated labels at https://chufangao.github.io/CTOD, with regular updates to support research on clinical trial outcomes and inform data-driven improvements in drug development.

==> main-paper.tex <==
% \documentclass[11pt]{article}

% % Language setting
% % Replace `english' with e.g. `spanish' to change the document language
% % \usepackage[english]{babel}
% % \usepackage{ctex}
% \usepackage{amssymb}
% \usepackage{amsmath}
% \usepackage{pdfpages}
% \usepackage{caption}
% % Set page size and margins
% % Replace `letterpaper' with `a4paper' for UK/EU standard size
% \usepackage[letterpaper,top=2cm,bottom=2cm,left=3cm,right=3cm,marginparwidth=1.75cm]{geometry}

% % Useful packages
% \usepackage{amsmath}
% \usepackage{graphicx}
% \usepackage[colorlinks=true, linkcolor=black, citecolor=blue]{hyperref}
% % \usepackage{lineno}
% \usepackage{color}
% \usepackage{xcolor}
% \usepackage{multirow}
% \usepackage{booktabs}
% \usepackage{xspace}
% \usepackage{setspace}
% \usepackage[superscript]{cite}
% \usepackage{float}

% \newcommand{\ZX}[1]{{\bf\color{red}[{ZX: #1}]}}
% \newcommand{\revise}[1]{{\color{red}{#1}}}


% \usepackage{graphicx} % For including graphics
% \usepackage{caption}  % For caption customization

% \usepackage{enumitem}
% \newcounter{suppfigure}
% \renewcommand{\thesuppfigure}{\arabic{suppfigure}} % S1, S2, S3...




% \usepackage{titletoc}
% \newcommand\DoToC{%
%   \startcontents
%   \printcontents{}{1}{\textbf{Contents}\vskip3pt\hrule\vskip5pt}
%   \vskip3pt\hrule\vskip5pt
% }
% \newcommand{\mycomment}[1]{}
% % \newcommand{\method}{\text{CTO}\xspace}
% \newcommand{\andy}[1]{{\small\color{red}{\bf andy:} #1}}
% \newcommand{\trisha}[1]{{\small\color{violet}{\bf Trisha:} #1}}
% \newcommand{\jathu}[1]{{\small\color{blue}{\bf Jathu:} #1}}

% \makeatletter
% \renewcommand{\maketitle}{\bgroup\setlength{\parindent}{0pt}
% \begin{flushleft}
%   \textbf{\@title}

%   \@author
% \end{flushleft}\egroup
% }
% \makeatother


% %\title{Automatically Labeling \$200B Life-Saving Datasets: A Large Clinical Trial Outcome Benchmark}
% \title{Automatically Labeling Clinical Trial Outcomes: A Large-Scale Benchmark for Drug Development}

% % The \author macro works with any number of authors. There are two commands
% % used to separate the names and addresses of multiple authors: \And and \AND.
% %
% % Using \And between authors leaves it to LaTeX to determine where to break the
% % lines. Using \AND forces a line break at that point. So, if LaTeX puts 3 of 4
% % authors names on the first line, and the last on the second line, try using
% % \AND instead of \And before the third author name.

% \author{Chufan Gao$^{*}$, Jathurshan Pradeepkumar$^{*}$, Trisha Das$^{*}$, Shivashankar Thati and \\ Jimeng Sun\\
% Department of Computer Science, University of Illinois Urbana-Champaign, Urbana, IL, USA \\
% $^*$ Equal contribution \\
% Corresponding author: \texttt{jimeng@illinois.edu}}




% % \author{%
% %   Chufan Gao\thanks{Equal contribution} \\
% %   Department of Computer Science\\
% %   University of Illinois Urbana-Champaign\\
% %   \texttt{chufan2@illinois.edu} \\
% %   % examples of more authors
% %   \And
% %   Jathurshan Pradeepkumar$^*$ \\
% %   Department of Computer Science\\
% %   University of Illinois Urbana-Champaign\\
% %   \texttt{jp65@illinois.edu} \\
% %   \And
% %   Trisha Das$^*$ \\
% %   Department of Computer Science\\
% %   University of Illinois Urbana-Champaign\\
% %   \texttt{trishad2@illinois.edu} \\
% %   \And
% %   Shivashankar Thati \\
% %   University of Illinois Urbana-Champaign \\
% %   \texttt{ssthati@outlook.com} \\
% %   % \texttt{email} \\
% %   \And
% %   Jimeng Sun \\
% %   Department of Computer Science\\
% %   Carle Illinois College of Medicine \\
% %   University of Illinois Urbana-Champaign\\
% %   \texttt{jimeng@illinois.edu} \\
% %   % \And
% %   % Coauthor \\
% %   % Affiliation \\
% %   % Address \\
% %   % \texttt{email} \\
% %   % \And
% %   % Coauthor \\
% %   % Affiliation \\
% %   % Address \\
% %   % \texttt{email} \\
% % }


% \begin{document}

% \maketitle
% % \linenumbers
% % \begin{abstract}



% % % The global cost of drug discovery and development exceeds \$200 billion annually. The main results of drug discovery and development are the outcomes of clinical trials, which directly influence the regulatory approval of new drug candidates and ultimately affect patient outcomes. Despite their significance, large-scale, high-quality clinical trial outcome data are not readily available to the public.
% % % This paper introduces the Clinical Trial Outcome (\method) dataset, the first large-scale, fully reproducible, open-source dataset of clinical trial outcomes, generated from an extensive knowledge base. This knowledge base incorporates weakly supervised labels that connect and contextualize multiple data sources, including trial phase transitions, large language model (LLM) interpretations of trial-related publications, sentiment analyses from news headlines, stock prices of sponsoring companies, and other trial-specific metrics.
% % % Our comprehensive labeling pipeline applies these weakly supervised sources to produce high-quality trial outcome labels. Validated against previously published human-annotated outcomes, this pipeline achieves an impressive 94 F1 score for Phase 3 trials and 91 across all phases. To support ongoing research, we provide monthly updates to the labeling process, knowledge base, and source code, along with a curated benchmark set of 10,140 recent trials completed between 2020-2024. This resource aims to enhance the reproducibility and accuracy of predictive models in clinical research.

% % %=$0.91$.

% % %Additionally, \method\ enables the unprecedented calculation of all trial outcomes, making it the first to identify a distribution shift in trials caused by COVID-19 empirically. This highlights the necessity for continuous automatic updates of outcome prediction models to adapt to changing circumstances in the clinical trial landscape.


% % % \method\ shows agreement against published trial outcome results, achieving promising results. Specifically, the combined \method\ labels demonstrated significant agreement with a supervised clinical trial outcome dataset, TOP (achieving 78 F1 on Phase 3 trials).
% % % \andy{make sure that we emphasize that we're the first to find this covid distribution shift. This is why we need continual automatic update of outcome labels. Emphasize don't need human annotators, so this is possible.}
% % \end{abstract}

% %TC:ignore
% \input{Context/Abstract}
% %TC:endignore

% \newpage
% \input{Context/Introduction}
% \input{Context/Method}

% \input{Context/Results}
% \input{Context/Discussion}

 








% % \paragraph{Agreement with Supervised TOP}
% % We construct our dataset such that the TOP test dataset is completely included within our test dataset. I.e. the start dates of the test set are after January 1, 2014, while the completion dates of the train/validation set are before January 1, 2014.


% % \section{Analysis and Experiments}

% %\subsection{Analysis of Trials Success by Overall Status}
% %Figure \ref{fig:normalized_stacked_bar}
% % \subsection{Which Labels Actually Matter?}





% % \begin{ack}

% %TC:ignore
% \paragraph{Acknowledgement}
% This work was supported by NSF award SCH-2205289, SCH-2014438, and IIS-2034479.
% % \end{ack}


% \bibliography{custom}
% \bibliographystyle{naturemag}
% %TC:endignore

% % \appendix
% % \mycomment{
% % \section{All Labeling Functions}
% % \begin{enumerate}
% %     \item Recruitment or safety reasons - easy (JP)
    
% %     \item Number of Amendments to the trial -(trisha) \andy{done}
    
% %     \item Whether trial was completed within time, date extension - projected completion vs actual completion? \andy{done}
    
% %     \item \texttt{were\_results\_reported} feature \andy{done}
    
% %     \item Patient Dropout, number of patients, number of sites, number of sponsors \andy{done}
    
% %     % \item Clinical Significance?

% %     \item Statistical and clinical significance of efficacy and safety endpoints - p-values \andy{done}
    
% %     \item GPT decision of Pubmed abstracts/conclusions (even existence of papers). Additionally, extract results, e.g., \textit{Results: As of the data cutoff on 17 June 2020, 68 patients were enrolled, and 59 were treated. Among the 58 efficacy-evaluable patients, the primary endpoint of 3-month ORR was 60.3\% (95\% CI, 46.6-73.0), excluding the null hypothesis rate of 20\%. Any grade and severe grade CRS occurred in 47.5\% and 5.1\%, respectively, and any grade and severe grade neurotoxicity events occurred in 20.3\% and 5.1\%.} (JP). 
    
% %     \item Momentary increase or decrease in company stock price in response to clinical trial results. \cite{aliper2023prediction}, \url{https://github.com/ranaroussi/yfinance} (Note: We should also predict stock prices directly) \andy{lf done}

% %     \item News datasets \url{https://github.com/Zdong104/FNSPID_Financial_News_Dataset}, headlines datasets, linked the stock prices We follow the methodology of \citet{dong2024fnspid} - Andy
    
% %     \item Company decision to transition drug program to phase III, official FDA-approved drugs for phase II (JP, trial linkage)
    

% %     \item total number of deaths, total number of subjects affected by serious adverse events, total number of subjects affected by any adverse events. (Trisha) \andy{done}

% %     \item \url{https://fda.gov/drugs/drug-approvals-and-databases/orange-book-data-files}
% % \end{enumerate}}

% % \newpage
% % \section*{Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% % The checklist follows the references.  Please
% % read the checklist guidelines carefully for information on how to answer these
% % questions.  For each question, change the default \answerTODO{} to \answerYes{},
% % \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% % justification to your answer}, either by referencing the appropriate section of
% % your paper or providing a brief inline description.  For example:
% % \begin{itemize}
% %   \item Did you include the license to the code and datasets? \answerYes{See Section .}
% %   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
% %   \item Did you include the license to the code and datasets? \answerNA{}
% % \end{itemize}
% % Please do not modify the questions and only use the provided macros for your
% % answers.  Note that the Checklist section does not count towards the page
% % limit.  In your paper, please delete this instructions block and only keep the
% % Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

% % \begin{enumerate}

% % \item For all authors...
% % \begin{enumerate}
% %   \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
% %     \answerYes{}
% %   \item Did you describe the limitations of your work?
% %     \answerYes{} See Conclusion
% %   \item Did you discuss any potential negative societal impacts of your work?
% %     \answerYes{}
% %   \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
% %     \answerYes{}
% % \end{enumerate}

% % \item If you are including theoretical results...
% % \begin{enumerate}
% %   \item Did you state the full set of assumptions of all theoretical results?
% %     \answerNA{}
% % 	\item Did you include complete proofs of all theoretical results?
% %     \answerNA{}
% % \end{enumerate}

% % \item If you ran experiments (e.g. for benchmarks)...
% % \begin{enumerate}
% %   \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
% %     \answerYes{}
% %   \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
% %     \answerYes{}
% % 	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
% %     \answerYes{}
% % 	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
% %     \answerYes{}
% % \end{enumerate}

% % \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
% % \begin{enumerate}
% %   \item If your work uses existing assets, did you cite the creators?
% %     \answerYes{}
% %   \item Did you mention the license of the assets?
% %     \answerYes{}
% %   \item Did you include any new assets either in the supplemental material or as a URL?
% %     \answerYes{}
% %   \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
% %     \answerNA{} We are using public data.
% %   \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
% %     \answerNA{}
% % \end{enumerate}

% % \item If you used crowdsourcing or conducted research with human subjects...
% % \begin{enumerate}
% %   \item Did you include the full text of instructions given to participants and screenshots, if applicable?
% %     \answerNA{}
% %   \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
% %     \answerNA{}
% %   \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
% %     \answerNA{}
% % \end{enumerate}

% % \end{enumerate}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% % \newpage



% \end{document}

==> old/old_test.tex <==
% \documentclass{article}


% % if you need to pass options to natbib, use, e.g.:
% %     \PassOptionsToPackage{numbers, compress}{natbib}
% % before loading neurips_2024


% % ready for submission
% \usepackage[nonatbib]{neurips_data_2024}


% % to compile a preprint version, e.g., for submission to arXiv, add add the
% % [preprint] option:
% %     \usepackage[preprint]{neurips_2024}


% % to compile a camera-ready version, add the [final] option, e.g.:
% %     \usepackage[final]{neurips_2024}


% % to avoid loading the natbib package, add option nonatbib:
% %    \usepackage[nonatbib]{neurips_2024}


% \usepackage[utf8]{inputenc} % allow utf-8 input
% \usepackage[T1]{fontenc}    % use 8-bit T1 fonts
% \usepackage{url}            % simple URL typesetting
% \usepackage{booktabs}       % professional-quality tables
% \usepackage{bm}
% \usepackage{amsmath}
% \usepackage{amsfonts}       % blackboard math symbols
% \usepackage{amssymb}% http://ctan.org/pkg/amssymb
% \usepackage{pifont}% http://ctan.org/pkg/pifont
% \newcommand{\cmark}{{\color{teal}\ding{51}}}
% \newcommand{\xmark}{{\color{red}\ding{55}}}%
% % \usepackage{nicefrac}       % compact symbols for 1/2, etc.
% \usepackage{microtype}      % microtypography
% \usepackage{xcolor}         % colors
% \usepackage{xspace}
% \usepackage{titletoc}
% \usepackage{graphicx}
% \usepackage{enumitem}
% \usepackage{wrapfig}
% \usepackage{multirow}

% \usepackage{subcaption}
% \usepackage{hyperref}       % hyperlinks

% \usepackage{titletoc}
% \newcommand\DoToC{%
%   \startcontents
%   \printcontents{}{1}{\textbf{Contents}\vskip3pt\hrule\vskip5pt}
%   \vskip3pt\hrule\vskip5pt
% }
% \newcommand{\mycomment}[1]{}
% \newcommand{\method}{\text{CTO}\xspace}
% \newcommand{\andy}[1]{{\small\color{red}{\bf andy:} #1}}
% \newcommand{\trisha}[1]{{\small\color{violet}{\bf Trisha:} #1}}

% % \title{\method: A Large-scale Clinical Trial Outcome Benchmark}

% \title{Automatically Labeling \$200B Life-Saving Datasets: A Large Clinical Trial Outcome Benchmark}

% % The \author macro works with any number of authors. There are two commands
% % used to separate the names and addresses of multiple authors: \And and \AND.
% %
% % Using \And between authors leaves it to LaTeX to determine where to break the
% % lines. Using \AND forces a line break at that point. So, if LaTeX puts 3 of 4
% % authors names on the first line, and the last on the second line, try using
% % \AND instead of \And before the third author name.


% \author{%
%   Chufan Gao\thanks{Equal contribution} \\
%   Department of Computer Science\\
%   University of Illinois Urbana-Champaign\\
%   \texttt{chufan2@illinois.edu} \\
%   % examples of more authors
%   \And
%   Jathurshan Pradeepkumar$^*$ \\
%   Department of Computer Science\\
%   University of Illinois Urbana-Champaign\\
%   \texttt{jp65@illinois.edu} \\
%   \And
%   Trisha Das$^*$ \\
%   Department of Computer Science\\
%   University of Illinois Urbana-Champaign\\
%   \texttt{trishad2@illinois.edu} \\
%   \And
%   Shivashankar Thati \\
%   University of Illinois Urbana-Champaign \\
%   \texttt{ssthati@outlook.com} \\
%   % \texttt{email} \\
%   \And
%   Jimeng Sun \\
%   Department of Computer Science\\
%   Carle Illinois College of Medicine \\
%   University of Illinois Urbana-Champaign\\
%   \texttt{jimeng@illinois.edu} \\
%   % \And
%   % Coauthor \\
%   % Affiliation \\
%   % Address \\
%   % \texttt{email} \\
%   % \And
%   % Coauthor \\
%   % Affiliation \\
%   % Address \\
%   % \texttt{email} \\
% }


% \begin{document}

% \maketitle

% \begin{abstract}
% The drug discovery and development process is characterized by high risk and frequent failures at various stages, including disease modeling, target discovery, and clinical trials. Accurate prediction of clinical trial outcomes can significantly improve this process by prioritizing therapeutic programs with a higher likelihood of success, ultimately benefiting patients. This paper introduces \method, an aggregated dataset of clinical trial outcomes derived from multiple sources of weakly supervised labels, eliminating the need for human annotators. Sources include large language model (LLM) interpretations of trial-related documents, news headline sentiments, stock prices of trial sponsors, subsequent trial linkages, and other signals such as patient dropout rates and adverse events.
% \method shows strong agreement with supervised clinical trial outcomes from the TOP dataset, with an average F1 score difference of \andy{x}. Additionally, \method enables the unprecedented calculation of all trial outcomes, making it the first to empirically identify a distribution shift in trials caused by COVID-19. This highlights the necessity for continuous automatic updates of outcome prediction models.
% % \method shows agreement against published trial outcome results, achieving promising results. Specifically, the combined \method labels demonstrated significant agreement with a supervised clinical trial outcome dataset, TOP (achieving 78 F1 on Phase 3 trials).
% % Furthermore, \method provides code for all weakly supervised labels in a reproducible format such that predicted labels for new trials may be calculated at will. Additionally, we aggregate trial-related data such as ICD Coding, drug mapping, and publications to enable reproducibility as well as secondary applications of stock price and trial linkage prediction. We make all of our code and data available at \url{https://github.com/chufangao/ctod}.
% % \andy{make sure that we emphasize that we're the first to find this covid distribution shift. This is why we need continual automatic update of outcome labels. Emphasize don't need human annotators, so this is possible.}
% \end{abstract}


% \section{intro}
% \subsection{Results on Pre-2020 Split vs Post-2020 Split}
% \begin{table}[ht]
% \centering
% \caption{Performance of baselines on both data splits of \method. The average difference for pre- and post-2020 is 0.108 F1, 0.181 PRAUC, and 0.011 ROCAUC.}
% \label{tab:prevspost}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{ccccc|ccc}
%  &  & \multicolumn{3}{c}{Pre-2020 Split} & \multicolumn{3}{c}{Post-2020 Split} \\
% Phase & Model & F1 & PRAUC & ROCAUC & F1 & PRAUC & ROCAUC \\ \toprule
% \multirow{7}{*}{I} & SVM & $0.486_{\pm0.015}$ & $0.479_{\pm0.017}$ & $0.639_{\pm0.012}$ & $0.419_{\pm0.013}$ & $0.366_{\pm0.015}$ & $0.647_{\pm0.010}$ \\
%  & XGBoost & $0.500_{\pm0.014}$ & $0.495_{\pm0.018}$ & $0.637_{\pm0.012}$ & $0.404_{\pm0.013}$ & $0.364_{\pm0.015}$ & $0.625_{\pm0.011}$ \\
%  & MLP & $0.502_{\pm0.015}$ & $0.479_{\pm0.016}$ & $0.637_{\pm0.012}$ & $0.388_{\pm0.011}$ & $0.326_{\pm0.013}$ & $0.601_{\pm0.008}$ \\
%  & RF & $0.496_{\pm0.016}$ & $0.504_{\pm0.017}$ & $0.661_{\pm0.012}$ & $0.419_{\pm0.012}$ & $0.367_{\pm0.013}$ & $0.658_{\pm0.008}$ \\
%  & LR & $0.514_{\pm0.013}$ & $0.490_{\pm0.018}$ & $0.650_{\pm0.011}$ & $0.427_{\pm0.011}$ & $0.369_{\pm0.014}$ & $0.650_{\pm0.009}$ \\
%  & BioBERT & $0.527_{\pm0.009}$ & $0.474_{\pm0.013}$ & $0.633_{\pm0.009}$ & $0.444_{\pm0.008}$ & $0.351_{\pm0.009}$ & $0.648_{\pm0.008}$ \\
%  & PubMedBERT & $0.544_{\pm0.015}$ & $0.445_{\pm0.014}$ & $0.617_{\pm0.012}$ & $0.456_{\pm0.008}$ & $0.312_{\pm0.007}$ & $0.618_{\pm0.007}$ \\ \midrule
% \multirow{7}{*}{II} & SVM & $0.577_{\pm0.012}$ & $0.611_{\pm0.016}$ & $0.658_{\pm0.011}$ & $0.455_{\pm0.009}$ & $0.423_{\pm0.013}$ & $0.658_{\pm0.008}$ \\
%  & XGBoost & $0.599_{\pm0.012}$ & $0.617_{\pm0.016}$ & $0.651_{\pm0.011}$ & $0.441_{\pm0.009}$ & $0.412_{\pm0.011}$ & $0.629_{\pm0.007}$ \\
%  & MLP & $0.545_{\pm0.010}$ & $0.574_{\pm0.013}$ & $0.606_{\pm0.010}$ & $0.437_{\pm0.009}$ & $0.375_{\pm0.011}$ & $0.604_{\pm0.008}$ \\
%  & RF & $0.561_{\pm0.012}$ & $0.609_{\pm0.016}$ & $0.643_{\pm0.011}$ & $0.445_{\pm0.009}$ & $0.398_{\pm0.010}$ & $0.637_{\pm0.007}$ \\
%  & LR & $0.602_{\pm0.011}$ & $0.622_{\pm0.015}$ & $0.666_{\pm0.010}$ & $0.468_{\pm0.011}$ & $0.427_{\pm0.011}$ & $0.663_{\pm0.007}$ \\
%  & BioBERT & $0.599_{\pm0.008}$ & $0.637_{\pm0.018}$ & $0.677_{\pm0.009}$ & $0.495_{\pm0.007}$ & $0.416_{\pm0.012}$ & $0.666_{\pm0.005}$ \\
%  & PubMedBERT & $0.626_{\pm0.009}$ & $0.569_{\pm0.012}$ & $0.630_{\pm0.007}$ & $0.501_{\pm0.009}$ & $0.360_{\pm0.009}$ & $0.626_{\pm0.005}$ \\ \midrule
% \multirow{7}{*}{III} & SVM & $0.639_{\pm0.013}$ & $0.708_{\pm0.015}$ & $0.681_{\pm0.012}$ & $0.545_{\pm0.012}$ & $0.521_{\pm0.015}$ & $0.676_{\pm0.010}$ \\
%  & XGBoost & $0.666_{\pm0.013}$ & $0.713_{\pm0.018}$ & $0.686_{\pm0.013}$ & $0.538_{\pm0.012}$ & $0.506_{\pm0.015}$ & $0.664_{\pm0.009}$ \\
%  & MLP & $0.614_{\pm0.014}$ & $0.683_{\pm0.016}$ & $0.648_{\pm0.012}$ & $0.509_{\pm0.011}$ & $0.458_{\pm0.014}$ & $0.626_{\pm0.010}$ \\
%  & RF & $0.619_{\pm0.015}$ & $0.718_{\pm0.017}$ & $0.687_{\pm0.014}$ & $0.511_{\pm0.012}$ & $0.491_{\pm0.013}$ & $0.661_{\pm0.009}$ \\
%  & LR & $0.659_{\pm0.013}$ & $0.722_{\pm0.016}$ & $0.693_{\pm0.013}$ & $0.551_{\pm0.011}$ & $0.519_{\pm0.014}$ & $0.678_{\pm0.009}$ \\
%  & BioBERT & $0.691_{\pm0.011}$ & $0.740_{\pm0.013}$ & $0.736_{\pm0.010}$ & $0.559_{\pm0.012}$ & $0.523_{\pm0.018}$ & $0.683_{\pm0.009}$ \\
%  & PubMedBERT & $0.692_{\pm0.013}$ & $0.650_{\pm0.012}$ & $0.671_{\pm0.012}$ & $0.577_{\pm0.010}$ & $0.452_{\pm0.011}$ & $0.649_{\pm0.007}$ \\ \bottomrule
% \end{tabular} 
% \vspace{-1em}
% }
% \end{table}
% We additionally show results from both pre- and post-2020 splits in Table~\ref{tab:prevspost}. The pre-2020 split shows generally higher performance across all metrics and phases compared to the post-2020 split, indicating that the pre-2020 data is easier to predict. The decline in performance post-2020 can be attributed to the complexities and disruptions introduced by the COVID-19 pandemic, which affected clinical trial operations and outcomes. Overall, these observations suggest that the pre-2020 data offers a more stable and predictable environment for clinical trial outcome prediction and that post-2020 data should require additional consideration.



% \subsection{Results on TOP (All Drugs)}
% \label{app:top_extended}

% In this section, we run comparisons of an extended training set--now selecting all interventional small molecule drug trials with completion dates before 2014. The sizes of our train, validation, and test splits are 47,080, 901, and 3165 respectively, with training and validation mined from \method (trials completed $<2014$ as per TOP \cite{fu2022hint}). We tested on the TOP test data. We demonstrate F1, PR-AUC, and ROC-AUC scores for all baseline models in table \ref{tab:vstop}. 
% % \subsection{Baselines}
% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=\linewidth]{figures/CTOD_vs_TOP_old.pdf}
%     \caption{Results on TOP test data split. The specific values can be found in Table~\ref{tab:vstop} in the Appendix. The average difference between TOP and \method is 0.048 F1,  0.077 PRAUC, and 0.098 ROCAUC.}
%     \label{fig: CTOD vs TOP} 
%     \vspace{-1em}
% \end{figure}

% \begin{table}[ht]
% \centering
% \caption{On TOP. Train/Valid/Test split is 47,080 / 901 / 3,165. The average difference between TOP and \method is 0.048 F1,  0.077 PRAUC, and 0.098 ROCAUC.}
% \label{tab:vstop}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{ccccc|ccc}
%  &  & \multicolumn{3}{c}{TOP} & \multicolumn{3}{c}{CTOD} \\
% Phase & Model & F1 & PRAUC & ROCAUC & F1 & PRAUC & ROCAUC \\ \toprule
% \multirow{7}{*}{phase 1} & SVM & $0.632_{\pm0.019}$ & $0.645_{\pm0.028}$ & $0.592_{\pm0.023}$ & $0.563_{\pm0.019}$ & $0.608_{\pm0.026}$ & $0.529_{\pm0.019}$ \\
%  & XGBoost & $0.630_{\pm0.020}$ & $0.637_{\pm0.025}$ & $0.596_{\pm0.021}$ & $0.586_{\pm0.021}$ & $0.584_{\pm0.024}$ & $0.527_{\pm0.024}$ \\
%  & MLP & $0.585_{\pm0.023}$ & $0.636_{\pm0.028}$ & $0.575_{\pm0.022}$ & $0.566_{\pm0.022}$ & $0.594_{\pm0.024}$ & $0.529_{\pm0.022}$ \\
%  & RF & $0.641_{\pm0.024}$ & $0.682_{\pm0.028}$ & $0.623_{\pm0.024}$ & $0.528_{\pm0.022}$ & $0.558_{\pm0.024}$ & $0.492_{\pm0.023}$ \\
%  & LR & $0.656_{\pm0.018}$ & $0.669_{\pm0.028}$ & $0.631_{\pm0.021}$ & $0.584_{\pm0.021}$ & $0.613_{\pm0.030}$ & $0.529_{\pm0.024}$ \\
%  & BioBERT & $0.653_{\pm0.017}$ & $0.674_{\pm0.014}$ & $0.622_{\pm0.021}$ & $0.567_{\pm0.023}$ & $0.563_{\pm0.023}$ & $0.504_{\pm0.027}$ \\
%  & PubMedBERT & $0.597_{\pm0.017}$ & $0.609_{\pm0.016}$ & $0.596_{\pm0.019}$ & $0.593_{\pm0.027}$ & $0.572_{\pm0.023}$ & $0.528_{\pm0.025}$ \\ \midrule
% \multirow{7}{*}{phase 2} & SVM & $0.672_{\pm0.011}$ & $0.664_{\pm0.017}$ & $0.626_{\pm0.013}$ & $0.613_{\pm0.013}$ & $0.578_{\pm0.017}$ & $0.529_{\pm0.014}$ \\
%  & XGBoost & $0.659_{\pm0.013}$ & $0.675_{\pm0.016}$ & $0.627_{\pm0.014}$ & $0.598_{\pm0.014}$ & $0.565_{\pm0.020}$ & $0.512_{\pm0.015}$ \\
%  & MLP & $0.615_{\pm0.014}$ & $0.640_{\pm0.017}$ & $0.599_{\pm0.014}$ & $0.611_{\pm0.012}$ & $0.595_{\pm0.018}$ & $0.542_{\pm0.015}$ \\
%  & RF & $0.675_{\pm0.011}$ & $0.690_{\pm0.016}$ & $0.643_{\pm0.014}$ & $0.574_{\pm0.014}$ & $0.539_{\pm0.017}$ & $0.475_{\pm0.014}$ \\
%  & LR & $0.674_{\pm0.013}$ & $0.697_{\pm0.017}$ & $0.648_{\pm0.012}$ & $0.626_{\pm0.012}$ & $0.579_{\pm0.017}$ & $0.528_{\pm0.013}$ \\
%  & BioBERT & $0.669_{\pm0.014}$ & $0.694_{\pm0.017}$ & $0.647_{\pm0.010}$ & $0.611_{\pm0.001}$ & $0.574_{\pm0.017}$ & $0.508_{\pm0.011}$ \\
%  & PubMedBERT & $0.644_{\pm0.009}$ & $0.612_{\pm0.008}$ & $0.600_{\pm0.010}$ & $0.595_{\pm0.011}$ & $0.561_{\pm0.013}$ & $0.509_{\pm0.010}$ \\ \midrule
% \multirow{7}{*}{phase 3} & SVM & $0.813_{\pm0.010}$ & $0.876_{\pm0.012}$ & $0.700_{\pm0.018}$ & $0.788_{\pm0.010}$ & $0.782_{\pm0.015}$ & $0.595_{\pm0.021}$ \\
%  & XGBoost & $0.815_{\pm0.010}$ & $0.849_{\pm0.015}$ & $0.674_{\pm0.017}$ & $0.789_{\pm0.010}$ & $0.799_{\pm0.017}$ & $0.597_{\pm0.019}$ \\
%  & MLP & $0.762_{\pm0.011}$ & $0.848_{\pm0.012}$ & $0.650_{\pm0.017}$ & $0.769_{\pm0.011}$ & $0.780_{\pm0.016}$ & $0.559_{\pm0.020}$ \\
%  & RF & $0.830_{\pm0.009}$ & $0.858_{\pm0.013}$ & $0.675_{\pm0.015}$ & $0.746_{\pm0.011}$ & $0.782_{\pm0.017}$ & $0.562_{\pm0.020}$ \\
%  & LR & $0.828_{\pm0.008}$ & $0.887_{\pm0.010}$ & $0.725_{\pm0.014}$ & $0.802_{\pm0.011}$ & $0.782_{\pm0.019}$ & $0.592_{\pm0.020}$ \\
%  & BioBERT & $0.832_{\pm0.010}$ & $0.850_{\pm0.016}$ & $0.662_{\pm0.018}$ & $0.791_{\pm0.012}$ & $0.808_{\pm0.022}$ & $0.592_{\pm0.025}$ \\
%  & PubMedBERT & $0.824_{\pm0.009}$ & $0.808_{\pm0.015}$ & $0.646_{\pm0.014}$ & $0.791_{\pm0.013}$ & $0.774_{\pm0.013}$ & $0.565_{\pm0.021}$ \\ \bottomrule
% \end{tabular}
% }
% \end{table}

% We see that from Table~\ref{tab:vstop} and Figure~\ref{fig: CTOD vs TOP} that our data is still close. However, SPOT and HINT perform quite badly on the extended dataset. We hypothesize that this is because both these models, due to their complexity tend to overfit to the TOP train split. However, simple baselines such as SVM and LR simply cannot overfit, and therefore better preserve the generalizability. Further investigation is required to fully analyze the distribution shift between the TOP training set and the set of all interventional drug trials.

% \andy{add bad SPOT AND HINT results here}

% \subsection{Additional Contributions}
% % \andy{potential Appendix}

% \paragraph{Additional Feature Collection}
% To run the baselines, we needed to collect ICD codes for diseases and SMILES strings \cite{weininger1988smiles} for drugs. We collected \textbf{ICD10 codes} for the diseases from the NIH Clinical Table Search Service\footnote{\url{https://clinicaltables.nlm.nih.gov/}}\cite{fu2022hint}. 
% % We slightly modified their code from \url{https://github.com/futianfan/clinical-trial-outcome-prediction/blob/main/benchmark/disease2icd.py} to accommodate cases that HINT cannot handle.
% We additionally collected \textbf{SMILES} (Simplified Molecular Input Line Entry System) strings for drugs from DrugBank 
% % \url{https://go.drugbank.com/releases/latest}. 
% We also used NIH PubChem\footnote{PubChemPy API \url{https://pubchempy.readthedocs.io/en/latest/}} \cite{kim2018update, kim2015pug, kim2019programmatic} to collect the SMILES we could not find in DrugBank.

% \paragraph{Stock Trend Prediction}
% The trend of a stock price is the overall direction in which the price of the stock is moving over a specified period, derived from the historical price data \cite{fidelity_trend}. As discussed in \ref{sec:stock}, we calculated the slope of stock prices. We define trend as the direction of the slope, i.e., positive slope refers to positive trend, and negative slope refers to negative trend. We tried to predict the trend of stock price in the 7-day window starting from a clinical trial's completion date.  Table \ref{tab:stockpred} shows the scores for different ML models for stock trend prediction. We utilized phase, eligibility criteria, diseases, and drugs as features for predicting trend. We get embeddings of the features using BioBERT and use the embeddings as input to the different baseline methods of Table \ref{tab:stockpred}. 

% \begin{wraptable}{R}{.3\linewidth}
% \vspace{-1.25em}
% \centering
% \setlength{\tabcolsep}{1pt}
% \caption{Comparison of model performance metrics for stock trend prediction}
% \label{tab:stockpred}
% \resizebox{\linewidth}{!}{
% \Huge
% \begin{tabular}{ccccccc}
%     Model & Accuracy & ROC AUC & F1 Score \\
%     \toprule
%     LR & 0.5121 & 0.5314 & 0.5531  \\
%     MLP               & 0.5418 & 0.5202 & 0.6620  \\
%     SVM                & 0.5441 & 0.4878 & 0.6860 \\
%     RF      & 0.5040 & 0.5103 & 0.5377  \\
%     XGBoost            & 0.5013 & 0.5077 & 0.5340 \\
%     \bottomrule
% \end{tabular}
% }
% \vspace{-1em}
% \end{wraptable} 

% \paragraph{QA Dataset}

% In addition to the weak trial outcome labels, we provide a QA dataset on trial publications as an additional contribution. While obtaining LLM predictions on PubMed abstracts, we prompted the model to generate question-answer pairs from the given abstracts. The prompts for generating the QA pairs are provided in the supplementary material (Fig.~\ref{fig:LLM_prompts}). The answers are provided in both short-answer and multiple-choice formats. Examples can be found in the supplementary material (Fig~\ref{fig:GPT_response example} and ~\ref{fig:GPT_response example2}). This QA dataset offers valuable information about the trials, complementing the weak outcome labels. It can be used for various downstream tasks, such as question answering, information extraction, and knowledge base construction related to clinical trials.

% \subsection{Data Programming}
% \label{app:dp}
% The full data programming framework is detailed by Ratner et al. \cite{ratner2019training}. We introduce a small aspect of the framework below.
% At a high level, the aggregation of weakly supervised labeling functions (LFs) is framed as a dependency graph $G_{source}$ where each LF $\lambda_i$ is dependently conditioned on the true label $Y$. In our case, we assume conditional independence of all $\lambda_i | Y$. For this case, the dependency graphs will have observable cliques  $\bm{O} = \{\lambda_i, i \in n_{lf}\} \subset C$, where $n_{lf}$ is the number of labeling functions.

% From here, the covariance matrix of an observable subset of the cliques in $G_{source}$ is analyzed, leading to a matrix completion approach for recovering estimated accuracies $\mu$ (used in the final label model to predict $P(\bm{Y}|\bm{\lambda})$).

% Let $\mu = \mathbb{E}(\psi(C))$ where $\psi(C)$ is a vector of indicator random variables for all combinations of all but one of the labels emitted by each variable in clique C.

% The norm of the covariance of observed LFs cliques $O$ and separator set $S$ cliques $\bm{Cov}(\psi(O) \cup \psi(S))$ can be used to recover $\mu$. 

% \begin{align}
% & \bm{Cov}(\psi(O) \cup \psi(S)) = \Sigma =  \begin{bmatrix}
% \Sigma_{O} & \Sigma_{OS} \\
% \Sigma_{OS}^T & \Sigma_{S}
% \end{bmatrix}
% \end{align}
% Its inverse is:
% \begin{align}
% & K = \Sigma^{-1} =  \begin{bmatrix}
% K_{O} & K_{OS} \\
% K_{OS}^T & K_{S}
% \end{bmatrix}
% \end{align}
% Applying block matrix inversion, we get:
% $$K_O = \Sigma^{-1}_O + c \Sigma^{-1}_O \Sigma_{OS} \Sigma^T_{OS} \Sigma^{-1}_{O}$$
% $$c = (\Sigma_{S} - \Sigma^T_{OS} \Sigma^{-1}_{O} \Sigma_{OS})$$
% Let $z = \sqrt{z} \Sigma^{-1}_{O} \Sigma_{OS}$, then
% $$K_O = \Sigma^{-1}_O + zz^T$$
% Solving for $z$ can directly recover estimated accuracies from $\mu$ via Algorithm 1 in Ratner et al. \cite{ratner2019training}.

% % \subsection{Case Studies}
% % In this section, we will analyze a few of the predicted differences between TOP and CTOD.

% % \subsection{LLM Prompts}

% \subsection{Clinical Trial Metrics in Detail}
% \label{app:metrics}

% (1) Whether results were reported, (2) The number of sponsors, (3) The number of patients, (4) The patient dropout rate, (5) The number of sites or locations for the trial, (6) Whether the P-value $<$ 0.05, (7) The date at which the trial was last updated vs its completion date, (8) Number of deaths, (9) Number of serious adverse events, (10) Number of \textit{any} adverse events, (11) The status of the trial e.g. terminated/withdrawn/completed/etc, and finally, (12) The number of amendments made to the trial page.

% \begin{itemize}[leftmargin=*]
% \item \texttt{results\_reported}
% \item \texttt{num\_sponsors}
% \item \texttt{num\_patients}
% \item \texttt{patient\_drop}
% \item \texttt{sites}
% \item \texttt{pvalues}
% \item \texttt{update\_more\_recent}
% \item \texttt{death\_ae, serious\_ae, all\_ae}: Represents the number of deaths, serious adverse events, and total adverse events, respectively. The total number of adverse events (AEs), serious adverse events (SAEs), and deaths in a clinical trial can provide important safety information about the investigational treatment. However, the significance of these numbers depends on various factors, including the size and duration of the trial, the nature of the treatment, and the characteristics of the study population. 
% \item \texttt{status}

% \item \texttt{amendments}: Represents the number of trial amendments:
% Clinical trials must follow approved protocols \cite{ICH2016, MHRA2012}, but amendments may be required after regulatory approval to adjust protocols according to new requirements or insights. 
% We scraped record histories for each trial from \url{https://clinicaltrials.gov/} and calculated the total number of times a clinical trial has been amended. The number of amendments to a clinical trial protocol can provide some insights into the trial's progress and potential success, but it's not necessarily a direct indication of success or failure. Therefore, we consider the total number of amendments of trial as a weak label.

% \item \texttt{stock\_price}: Is positive if the sponsor stock price's 5-day moving average has a positive or negative slope. See Section~\ref{sec:stock}.

% \item \texttt{linkage}: Is positive if a trial was found to have any later-stage trials linked to it. See Section~\ref{sec:linkage}.

% \item \texttt{news\_headlines}: Is positive or negative depending on sentiment from any news headline related to the trial. See Section~\ref{sec:news}.

% \item \texttt{gpt}: Represents GPT3.5-turbo-0125's decisions on PubMed abstracts. See Section~\ref{sec:gpt}

% \end{itemize}

% \newpage
% \subsection{Labeling Function Statistics}
% Table~\ref{tab:all_lf_stats} represents a table of all statistics regarding the labeling functions we choose to implement. We note that the status LF is very rarely 1, and is mostly 0, as positive labels only occur 0.4\% of the time. This leads to F1 scores of 0 for certain phases in TOP where only 0 is predicted.

% \begin{table}[ht]
% \centering
% \caption{Table of all statistics of the different labeling functions that we consider for \method. Note that for Data Programming, the labeling function of -1 is no prediction. Positive Prop. refers to the positive percentage of all valid labels (i.e. $\frac{\#1}{\#1+\#0}$). Coverage indicates the proportion of all trials that the LF has predictions on. Pos. F1 and Neg. F1 represent F1 scores on positive and negative TOP labels for all phases.}
% \label{tab:all_lf_stats}
% \resizebox{\linewidth}{!}{
% \Huge
% \begin{tabular}{cccccc|cc|cc|cc}
%  &  &  &  &  &  & \multicolumn{2}{c}{Phase I} & \multicolumn{2}{c}{Phase II} & \multicolumn{2}{c}{Phase III} \\ \toprule
% Labeling Function & -1 & 0 & 1 & \begin{tabular}[c]{@{}c@{}}Positive\\ Prop.\end{tabular} & Coverage & Pos. F1 & Neg. F1 & Pos. F1 & Neg. F1 & Pos. F1 & Neg. F1 \\ \toprule
% results\_reported & 0 & 415614 & 61624 & 0.129 & 1.000 & 0.410 & 0.494 & 0.529 & 0.518 & 0.690 & 0.506 \\
% num\_sponsors & 0 & 321091 & 156147 & 0.327 & 1.000 & 0.367 & 0.440 & 0.366 & 0.527 & 0.315 & 0.411 \\
% num\_patients & 0 & 30831 & 30793 & 0.500 & 1.000 & 0.512 & 0.681 & 0.634 & 0.681 & 0.837 & 0.343 \\
% patient\_drop & 0 & 19191 & 18554 & 0.492 & 1.000 & 0.449 & 0.343 & 0.413 & 0.435 & 0.206 & 0.383 \\
% sites & 0 & 313131 & 113484 & 0.266 & 1.000 & 0.555 & 0.529 & 0.534 & 0.496 & 0.632 & 0.327 \\
% pvalues & 0 & 10855 & 10386 & 0.489 & 1.000 & 0.605 & 0.564 & 0.702 & 0.661 & 0.835 & 0.610 \\
% update\_more\_recent & 16868 & 230601 & 229769 & 0.499 & 0.965 & 0.241 & 0.616 & 0.165 & 0.667 & 0.077 & 0.501 \\
% death\_ae & 0 & 10326 & 51094 & 0.832 & 1.000 & 0.680 & 0.255 & 0.661 & 0.143 & 0.833 & 0.116 \\
% serious\_ae & 0 & 29213 & 32207 & 0.524 & 1.000 & 0.341 & 0.534 & 0.304 & 0.558 & 0.195 & 0.399 \\
% all\_ae & 0 & 30569 & 30851 & 0.502 & 1.000 & 0.268 & 0.402 & 0.191 & 0.474 & 0.134 & 0.389 \\
% status & 432907 & 44136 & 195 & 0.004 & 0.093 & 0.000 & 0.976 & 0.000 & 0.984 & 0.000 & 0.977 \\
% amendments & 0 & 10989 & 8895 & 0.447 & 1.000 & 0.625 & 0.256 & 0.627 & 0.363 & 0.699 & 0.279 \\
% stock\_price & 0 & 9386 & 10498 & 0.528 & 1.000 & 0.670 & 0.239 & 0.576 & 0.405 & 0.652 & 0.362 \\
% linkage & 0 & 116695 & 35355 & 0.233 & 1.000 & 0.538 & 0.492 & 0.559 & 0.591 & 0.698 & 0.508 \\
% news\_headlines & 76526 & 2421 & 8427 & 0.777 & 0.124 & 0.721 & 0.205 & 0.694 & 0.352 & 0.752 & 0.337 \\
% gpt & 519 & 93642 & 69831 & 0.427 & 0.997 & 0.728 & 0.604 & 0.763 & 0.723 & 0.845 & 0.708 \\ \bottomrule
% \end{tabular}

% }
% \end{table}

% % \newpage
% \subsection{Statistics on Trial Linkage}
% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=\textwidth]{figures/Trial_linkage_statistics.pdf}
%     \caption{Overview of the weak labels extracted from the trial linkage.}
%     \label{fig:trial_linkage_feat_ablation}
% \end{figure}

% \newpage
% \subsection{Statistics on LLM Predictions}
% \label{supplementary: Statistics on LLM Predictions}

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=\linewidth]{figures/LLM_predictions_figure.pdf}
%     \caption{Overview of the weak labels from LLM predictions on PubMed abstracts.}
%     \label{fig:LLM_predictions_statistics}
% \end{figure}

% \newpage
% \subsection{Statistics of \method dataset}
% \begin{figure}[ht]
%     \centering
%     \begin{subfigure}{0.49\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/all_completion_before_2020_phase.pdf}
%         \caption{All trials with completion dates before 2020}
%         % \label{fig:a}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.49\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/completion_dates_between_2020_to_2024_phase.pdf}
%         \caption{Trials completed between 2020 and 2024}
%         % \label{fig:b}
%     \end{subfigure}
%     \caption{Statistics of all \method labels}
%     \label{fig:overall_status_part1}
% \end{figure}

% \begin{figure}[ht]
%     \centering
%     \begin{subfigure}{0.49\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/pre_pie_chart_phase.pdf}
%         \caption{Pre-covid data (small molecules only)}
%         % \label{fig:c}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.49\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{figures/post_pie_chart_phase.pdf}
%         \caption{Post-covid data (small molecules only)}
%         % \label{fig:another}
%     \end{subfigure}
%     \caption{Distributions of phases in different splits of \method dataset}
%     \label{fig:overall_status_part2}
% \end{figure}
% The total number of clinical trials in our dataset is 479761. There are a total of 429796 clinical trials in our \method dataset after removing trials with no phase information. Figure~\ref{fig:overall_status_part1} and Figure~\ref{fig:overall_status_part2} show the proportions of phases in different splits of our dataset.  


% % \begin{figure}[ht]
% %     \centering
% %     \includegraphics[width=\linewidth]{figures/Mismatch labels between TOP and CTOD.pdf}
% %     \caption{Distribution of differences of the labels between the human-annotated TOP dataset and our CTOD dataset across phases and trial statuses. A good observation from these plots is that some of the terminated trials have been labeled as success in the TOP dataset, whereas ours have correctly identified them as failed trials.}
% %     \label{fig:Mismatch labels between TOP and CTOD}
% % \end{figure}
% % % \andy{we need to update these for pre and post as well, also we need to change to pdf}

% % commented out due to updating labels
% % \begin{figure}[ht]
% %     \centering
% %     \includegraphics[width=0.8\linewidth]{figures/normalized_stacked_bar_plot.png}
% %     \caption{Proportions of labels (failure: 0, success: 1) in each type of overall\_status in \method dataset}
% %     \label{fig:normalized_stacked_bar}
% % \end{figure}

% %\begin{figure}[ht]
%    % \centering
%    % \includegraphics[width=.9\linewidth]{figures/combined_pie_charts_with_legend.png}
%    % \caption{Proportions of Overall Status and Phases in the \method dataset}
%    % \label{fig:overall_status_pie_chart}
% %\end{figure}

% \newpage
% \subsection{Trial Linkage in Detail}
% \label{app:Trial_Linkage_Continued}
% \textbf{1. Search space selection:} We begin by filtering the trials from connected phases based on their completion dates relative to the start date of $x$, ensuring that any linkage candidate must have concluded before the commencement of $x$. Furthermore, we refine the search space by filtering for trials with similar intervention characteristics as $x$, such as 'Drug', 'Biological', 'Device', etc. This step increases the likelihood of identifying relevant and meaningful connections.
    
% \textbf{2. Retrieve top-K:} From the filtered search space $\mathbf{Z}$, we retrieve top-K most similar past trials to $x$. We extract key features and encode them into dense embedding to represent both $x$ and trials in the search space ($z_i \in Z$) as follows: $x = \{x_{\text{I}},x_{\text{C}},x_{\text{T}},x_{\text{S}},x_{\text{E}}\}$,  $z_i =  \{z^i_{\text{I}},z^i_{\text{C}},z^i_{\text{T}},z^i_{\text{S}},z^i_{\text{E}}\}$.

% Where the subscript $I$ denotes intervention or drug, $C$ denotes condition or targeted disease, $T$ denotes official trial title, $S$ denotes trial summary, and $E$ denotes eligibility criteria.  
    
% We excluded the lead sponsor as a feature to represent the trial for this task due to two reasons: 1) During progress from phases, the sponsorship often changes depending on their funding capacity, and 2) Based on our ablation given in supplementary~\ref{supplementary: Ablation on Features for Trial Linkage}, the inclusion of lead sponsor adversely impacted agreement between extracted weak labels and the TOP dataset. We utilized BiomedBERT \cite{gu2021domain} from HuggingFace to obtain dense embeddings for each feature. This model, previously named PubMedBERT, was pre-trained on PubMed abstracts and PubMedCentral full-texts. For lengthy features like `brief summary' and `eligibility criteria', we chunked them into 512-token segments, encoded them, and obtained the final embedding by mean pooling. Utilizing these embeddings, we performed a semantic search to obtain top-K ($K = 32$) similar trials using the cosine similarity score aggregated across features as follows:
% $\text{similarity}(x,z_i) = \sum_{i \in \mathbf{F}}\frac{x^i.z_j^i}{||x^i||||z_j^i||}
% $,
%     % \begin{equation}
%     %     \text{aggregated cos\_sim}(x,z_i) = \sum_{j \in \mathbf{F}}\frac{x^j.z_i^j}{||x^j||||z_i^j||}
%     % \end{equation}
% Where $\mathbf{F} =$ \{I,C,T,S,E\}. We convert the intervention name of drugs to their generic name based on the data from DrugBank\footnote{https://go.drugbank.com/} for standardization.

% \textbf{3. Predict linkage} Given the large search space of clinical trials, the initial retrieval may return irrelevant candidates. To mitigate this and predict the most probable previous phase candidate for $x$, we employ a re-ranking strategy using cross-encoders, which are pre-trained to predict the relevance of a retrieved passage given a query. We utilize a cross-encoder $g_{\theta}$ pre-trained on MS-MARCO \cite{nguyen2016ms}, a large information retrieval corpus based on user search queries from Bing. We provide feature pairs as input to the cross-encoder, obtaining and aggregating their scores across features before the final Sigmoid activation layer as follows: $\text{Cross-encoder score}(x,z_i) = \sum_{j \in \mathbf{F}}g_{\theta}(x^i,z^i_j)$.
%     % \begin{equation}
%     %     \text{Cross-encoder score}(x,z_i) = \sum_{j \in \mathbf{F}}g_{\theta}(x^j,z^j_i)
%     % \end{equation}
% Based on the cross-encoder scores, we predict the linkage by considering the trials with the highest positive cross-encoder scores as the most probable previous phase trials of $x$.


% \subsection{Ablation on Features for Trial Linkage}
% \label{supplementary: Ablation on Features for Trial Linkage}

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=.8\linewidth]{figures/F1_Comparison_Across_Features.png}
%     \caption{Ablation study on the use of different trial features to predict trial linkages and the agreement of their extracted weak labels with TOP human-annotated data labels using F1 scores.}
%     \label{fig:trial_linkage_feat_ablation2}
% \end{figure}

% \begin{table}[ht]
% \centering
% \caption{Results of the ablation study on the different combinations of trial features to predict trial linkages and the agreement of their extracted weak labels with TOP human-annotated data labels using F1 scores.}
% \label{tab:feat_comb_trial_linkage}
% \vspace{0.1cm}
% \resizebox{\linewidth}{!}{
% \begin{tabular}{c|c|c}
% Phase & Feature combination & F1
%  \\ \midrule
% \multirow{5}{*}{Phase 1} & Official title + Intervention & 0.645 \\
% & Official title + Intervention + Brief Summary & 0.6426 \textcolor{red}{$\downarrow$}\\
% & Official title + Intervention + Brief Summary + Eligibility & 0.6447\textcolor{green}{$\uparrow$}\\
% & Official title + Intervention + Brief Summary + Eligibility + Condition & 0.6532 \textcolor{green}{$\uparrow$}\\
% & Official title + Intervention + Brief Summary + Eligibility + Condition + Lead Sponsor & \textbf{0.6658} \textcolor{green}{$\uparrow$}\\ \midrule

% \multirow{5}{*}{Phase 2} & Official title + Intervention & 0.6027\\
% & Official title + Intervention + Brief Summary & 0.6042 \textcolor{green}{$\uparrow$} \\
% & Official title + Intervention + Brief Summary + Eligibility & 0.608 \textcolor{green}{$\uparrow$}\\
% & Official title + Intervention + Brief Summary + Eligibility + Condition & \textbf{0.6196} \textcolor{green}{$\uparrow$}\\
% & Official title + Intervention + Brief Summary + Eligibility + Condition + Lead Sponsor & 0.6189\textcolor{red}{$\downarrow$}\\ \midrule

% \multirow{5}{*}{Phase 3} & Official title + Intervention & 0.7323 \\
% & Official title + Intervention + Brief Summary & 0.7319\textcolor{red}{$\downarrow$}\\
% & Official title + Intervention + Brief Summary + Eligibility & 0.7379\textcolor{green}{$\uparrow$}\\
% & Official title + Intervention + Brief Summary + Eligibility + Condition & \textbf{0.7498}\textcolor{green}{$\uparrow$} \\
% & Official title + Intervention + Brief Summary + Eligibility + Condition + Lead Sponsor & 0.7384 \textcolor{red}{$\downarrow$}\\ \midrule

% \multirow{5}{*}{All} & Official title + Intervention & 0.6686\\
% & Official title + Intervention + Brief Summary & 0.6687\textcolor{green}{$\uparrow$}\\
% & Official title + Intervention + Brief Summary + Eligibility & 0.6737\textcolor{green}{$\uparrow$}\\
% & Official title + Intervention + Brief Summary + Eligibility + Condition & \textbf{0.6842}\textcolor{green}{$\uparrow$} \\
% & Official title + Intervention + Brief Summary + Eligibility + Condition + Lead Sponsor & 0.6796\textcolor{red}{$\downarrow$}\\ 
% \bottomrule
% \end{tabular}
% }
% \flushleft{\textcolor{red}{$\downarrow$} indicates that adding the feature decreased the performance.\\\textcolor{green}{$\uparrow$} indicates that adding the feature improved the performance.}

% \end{table}

% \newpage
% \subsection{Prompts for LLM Predictions on PubMed Abstracts}
% \label{supplementary: Prompts for LLM Predictions}
% We show an example of such a prompt in Figure~\ref{fig:LLM_prompts}.

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=\linewidth]{figures/LLM_prompts.pdf}
%     \caption{LLM Prompts.}
%     \label{fig:LLM_prompts}
% \end{figure}

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=\linewidth]{figures/GPT_response_example_1.pdf}
%     \caption{Example response from GPT-3.5.}
%     \label{fig:GPT_response example}
% \end{figure}

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=\linewidth]{figures/GPT_response_example_2.pdf}
%     \caption{Example response 2 from GPT-3.5.}
%     \label{fig:GPT_response example2}
% \end{figure}

% \end{document}
